Repairing Reward Functions with Feedback to Mitigate Reward Hacking

Human-designed reward functions for reinforcement learning (RL) agents are frequently misaligned with the humans' true, unobservable objectives, and thus act only as proxies. Optimizing for a misspecified proxy reward function often induces reward hacking, resulting in a policy misaligned with the human's true objectives. An alternative is to perform RL from human feedback, which involves learning a reward function from scratch by collecting human preferences over pairs of trajectories. However, building such datasets is costly. To address the limitations of both approaches, we propose Preference-Based Reward Repair (PBRR): an automated iterative framework that repairs a human-specified proxy reward function by learning an additive, transition-dependent correction term from preferences. A manually specified reward function can yield policies that are highly suboptimal under the ground-truth objective, yet corrections on only a few transitions may suffice to recover optimal performance. To identify and correct for those transitions, PBRR uses a targeted exploration strategy and a new preference-learning objective. We prove in tabular domains PBRR has a cumulative regret that matches, up to constants, that of prior preference-based RL methods. In addition, on a suite of reward-hacking benchmarks, PBRR consistently outperforms baselines that learn a reward function from scratch from preferences or modify the proxy reward function using other approaches, requiring substantially fewer preferences to learn high performing policies.

==> sections/future_theory_if_correction_sparse.tex <==
We next consider when there may be some benefits to leveraging a prior specified proxy function. 
%Theorems \ref{thm:known_trans_model_regret_bound} and \ref{thm:unknown_trans_model_regret_bound} gives tight regret guarantees when learning a reward function from preferences over trajectory pairs following Algorithm \ref{alg:exploration}. 
We can always decompose the ground-truth reward function $r$ into the initially provided proxy reward function component and an unknown correction term. % 

We now show that, when the proxy reward function already captures a high-dimensional part of $r$, the effective learning dimension is reduced to that of the correction term alone. As a consequence, repairing a proxy reward function using Algorithm \ref{alg:exploration} requires quadratically fewer preference queries than learning the entire reward function from scratch. This conclusion holds both for known and unknown transition dynamics, as formalized in Lemma~\ref{lem:residual-dim}, Corollary~\ref{cor:improvement-factor}, and the subsequent remark.



\begin{lemma}
\commentsh{NOTE: I need to redo this lemma I defined $C_1$ and $C_2$ incorrectly but the general claim should still hold}
\label{lem:residual-dim}
Assume Algorithm \ref{alg:exploration} and Assumptions \ref{asm:linear},\ref{asm:bounded} and \ref{asm:bounded_features}. 
Suppose the (unobservable) ground-truth reward function decomposes as
\[
r(\tau) \;=\; w_p^\top \phi_p(\tau) \;+\; w_\ell^\top \phi_\ell(\tau),
\]
where $w_p$ and $\phi_p:\Gamma\to\R^{d_p}$ are \emph{known} (i.e., the human-specified proxy reward function), $\phi_\ell:\Gamma\to\R^{d_\ell}$ is \emph{known}, and $w_\ell\in\R^{d_\ell}$ is \emph{unknown}. 
Let $d_{\mathrm{full}} := \dim\!\big(\mathrm{span}(\phi_p,\phi_\ell)\big)\in[\max\{d_p,d_\ell\},\,d_p{+}d_\ell]$.
\end{lemma}

% \noindent\textbf{Known transition dynamics.}

If transition dynamics are known, let $C_2 = C_1 ( \kappa \sqrt{\lambda} W + \sqrt{d}  + B W \sqrt{d} )$. If transition dynamics are unkown, let $C_2 = C_1  \left( 
\kappa \sqrt{d} + H^{3/2} \sqrt{|\mathcal{S}||\mathcal{A}| H} 
+ H |\mathcal{S}| \sqrt{|\mathcal{A}| H} 
\right)$. Algorithm \ref{alg:exploration}'s regret scales as $\;\widetilde{\mathcal O}(C_2\sqrt{Td})$ for problem-dependent constant $C_2$. The average-regret sample complexity to reach $\tfrac{R_T}{T}\le \varepsilon$ satisfies
\[
T^{\mathrm{full}}_\varepsilon \;=\; \widetilde{\mathcal O}\!\Big(\tfrac{(C_2 d_{\mathrm{full}})^2}{\varepsilon^2}\Big),
\qquad
T^{\mathrm{res}}_\varepsilon \;=\; \widetilde{\mathcal O}\!\Big(\tfrac{(C_2 d_\ell)^2}{\varepsilon^2}\Big),
\]
i.e., repairing a proxy reward function (learning $w_\ell$ with $w_p$ known) replaces $d_{\mathrm{full}}$ by $d_\ell$ throughout. 

\medskip
% \noindent\textbf{Unknown transition dynamics.}

\begin{proof}[Proof sketch]
Under the Bradley–Terry model, preferences over $(\tau_1,\tau_2)$ depend on the the difference in return:
\[
\langle \phi(\tau_1)-\phi(\tau_2),\,w^\star\rangle
\;=\;
\underbrace{\big(r_p(\tau_1)-r_p(\tau_2)\big)}_{\text{known offset}}
\;+\;
\langle \phi_\ell(\tau_1)-\phi_\ell(\tau_2),\, w_\ell^\star\rangle.
\]
The proxy reward function term $r_p(\tau_1)-r_p(\tau_2)$ is a fixed, known offset and introduces no unknown parameters in the preference likelihood; hence the only uncertainty is in $w_\ell$, and Algorithm \ref{alg:exploration}'s confidence sets (and thus the $d$ factor in the regret bounds) are governed by the \emph{unknown} dimension $d_\ell$, not by $d_{\mathrm{full}}$. Substituting $d\!\leftarrow\! d_\ell$ in the known/unknown-dynamics bounds yields the sample-complexity claims above; learning a reward function \emph{ab initio} uses $d=d_{\mathrm{full}}$. \qedhere \commentsh{(Assuming this lemma is true) do we need to go beyond this proof-sketch? }
\end{proof}
\begin{corollary}
\commentsh{My major concern here is that this is a bit hand-wavy because $C_2$ absorbs $\sqrt{d}$; let me know if that invalidates the argument.}
\label{cor:improvement-factor}
Under the conditions of Lemma~\ref{lem:residual-dim}, the ratio of sample complexities satisfies
\[
\frac{T^{\mathrm{full}}_\varepsilon}{T^{\mathrm{res}}_\varepsilon}
\;=\;
\widetilde{\Omega}\!\left(\left(\frac{d_{\mathrm{full}}}{d_\ell}\right)^{\!2}\right),
\]
so when $d_\ell\ll d_p$ (and hence typically $d_{\mathrm{full}}\approx d_p{+}d_\ell$), learning an additive correction term for an existing proxy reward function attains a quadratic-in-dimension reduction in the number of preference queries needed to reach a fixed target average regret.
\end{corollary}

\begin{remark}[Overlapping feature sets]
If $\mathrm{span}(\phi_\ell)\subseteq \mathrm{span}(\phi_p)$, then $d_{\mathrm{full}}=\max\{d_p,d_\ell\}=d_p$ and the improvement factor becomes $(d_p/d_\ell)^2$.
If the spans are disjoint, $d_{\mathrm{full}}=d_p{+}d_\ell$, yielding a factor $\big((d_p{+}d_\ell)/d_\ell\big)^2$.
\end{remark}


\medskip

